Decentralized Gradient Tracking with Local Steps

Gradient tracking (GT) is an algorithm designed for solving decentralized optimization problems over a network (such as training a machine learning model). A key feature of GT is a tracking mechanism that allows to overcome data heterogeneity between nodes. We develop a novel decentralized tracking mechanism, $K$-GT, that enables communication-efficient local updates in GT while inheriting the data-independence property of GT. We prove a convergence rate for $K$-GT on smooth non-convex functions and prove that it reduces the communication overhead asymptotically by a linear factor $K$, where $K$ denotes the number of local steps. We illustrate the robustness and effectiveness of this heterogeneity correction on convex and non-convex benchmark problems and on a non-convex neural network training task with the MNIST dataset.

==> journal/configuration/epfml_macros.tex <==
% math
\usepackage{amsmath,amsthm,amssymb}
\theoremstyle{plain}% Theorem-like structures provided by amsthm.sty
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{claim}[theorem]{Claim}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}

% math notations.
\providecommand{\lin}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

\providecommand{\refLE}[1]{\ensuremath{\stackrel{(\ref{#1})}{\leq}}}
\providecommand{\refEQ}[1]{\ensuremath{\stackrel{(\ref{#1})}{=}}}
\providecommand{\refGE}[1]{\ensuremath{\stackrel{(\ref{#1})}{\geq}}}
\providecommand{\refID}[1]{\ensuremath{\stackrel{(\ref{#1})}{\equiv}}}

% basec sets
\providecommand{\R}{\mathbb{R}} % Reals
\providecommand{\N}{\mathbb{N}} % Naturals

% random variables
\providecommand{\E}{{\mathbb E}}
\providecommand{\E}[1]{{\mathbb E}\left.#1\right. }        %expectation
\providecommand{\Eb}[1]{{\mathbb E}\left[#1\right] }       %expectation, with brackets
\providecommand{\EE}[2]{{\mathbb E}_{#1}\left.#2\right. }  %expectation  
\providecommand{\EEb}[2]{{\mathbb E}_{#1}\left[#2\right] } %expectation,  with brackets
\providecommand{\prob}[1]{{\rm Pr}\left[#1\right] }
\providecommand{\Prob}[2]{{\rm Pr}_{#1}\left[#2\right] }
\providecommand{\P}[1]{{\rm Pr}\left.#1\right. }
\providecommand{\Pb}[1]{{\rm Pr}\left[#1\right] }
\providecommand{\PP}[2]{{\rm Pr}_{#1}\left[#2\right] }
\providecommand{\PPb}[2]{{\rm Pr}_{#1}\left[#2\right] }
\providecommand{\derive}[2]{\frac{{\partial}{#1}}{\partial #2} }  %expectation  

% operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\Tr}{Tr}

% bold vectors
\providecommand{\0}{\mathbf{0}}
\providecommand{\1}{\mathbf{1}}
\renewcommand{\aa}{\mathbf{a}}
\providecommand{\bb}{\mathbf{b}}
\providecommand{\cc}{\mathbf{c}}
\providecommand{\dd}{\mathbf{d}}
\providecommand{\ee}{\mathbf{e}}
\providecommand{\ff}{\mathbf{f}}
\let\ggg\gg
\renewcommand{\gg}{\mathbf{g}}
\providecommand{\gv}{\mathbf{g}}
\providecommand{\hh}{\mathbf{h}}
\providecommand{\ii}{\mathbf{i}}
\providecommand{\jj}{\mathbf{j}}
\providecommand{\kk}{\mathbf{k}}
\let\lll\ll
\renewcommand{\ll}{\mathbf{l}}
\providecommand{\mm}{\mathbf{m}}
\providecommand{\nn}{\mathbf{n}}
\providecommand{\oo}{\mathbf{o}}
\providecommand{\pp}{\mathbf{p}}
\providecommand{\qq}{\mathbf{q}}
\providecommand{\rr}{\mathbf{r}}
\renewcommand{\ss}{\mathbf{s}}
\providecommand{\tt}{\mathbf{t}}
\providecommand{\uu}{\mathbf{u}}
\providecommand{\vv}{\mathbf{v}}
\providecommand{\ww}{\mathbf{w}}
\providecommand{\xx}{\mathbf{x}}
\providecommand{\yy}{\mathbf{y}}
\providecommand{\zz}{\mathbf{z}}
\providecommand{\unit}{\mathbf{1}}
\providecommand{\zero}{\mathbf{0}}
% bold matrices
\providecommand{\mA}{\mathbf{A}}
\providecommand{\mB}{\mathbf{B}}
\providecommand{\mC}{\mathbf{C}}
\providecommand{\mD}{\mathbf{D}}
\providecommand{\mE}{\mathbf{E}}
\providecommand{\mF}{\mathbf{F}}
\providecommand{\mG}{\mathbf{G}}
\providecommand{\mH}{\mathbf{H}}
\providecommand{\mI}{\mathbf{I}}
\providecommand{\mJ}{\mathbf{J}}
\providecommand{\mK}{\mathbf{K}}
\providecommand{\mL}{\mathbf{L}}
\providecommand{\mM}{\mathbf{M}}
\providecommand{\mN}{\mathbf{N}}
\providecommand{\mO}{\mathbf{O}}
\providecommand{\mP}{\mathbf{P}}
\providecommand{\mQ}{\mathbf{Q}}
\providecommand{\mR}{\mathbf{R}}
\providecommand{\mS}{\mathbf{S}}
\providecommand{\mT}{\mathbf{T}}
\providecommand{\mU}{\mathbf{U}}
\providecommand{\mV}{\mathbf{V}}
\providecommand{\mW}{\mathbf{W}}
\providecommand{\mX}{\mathbf{X}}
\providecommand{\mY}{\mathbf{Y}}
\providecommand{\mZ}{\mathbf{Z}}
\providecommand{\mLambda}{\boldsymbol{\Lambda}}
\providecommand{\mpi}{\boldsymbol{\pi}}
\providecommand{\malpha}{\boldsymbol{\alpha}}
\providecommand{\meta}{\boldsymbol{\eta}}
\providecommand{\mxi}{\boldsymbol{\xi}}
\providecommand{\mepsilon}{\boldsymbol{\epsilon}}
\providecommand{\mphi}{\boldsymbol{\phi}}

% caligraphic
\providecommand{\cA}{\mathcal{A}}
\providecommand{\cB}{\mathcal{B}}
\providecommand{\cC}{\mathcal{C}}
\providecommand{\cD}{\mathcal{D}}
\providecommand{\cE}{\mathcal{E}}
\providecommand{\cF}{\mathcal{F}}
\providecommand{\cG}{\mathcal{G}}
\providecommand{\cH}{\mathcal{H}}
\providecommand{\cI}{\mathcal{I}}
\providecommand{\cJ}{\mathcal{J}}
\providecommand{\cK}{\mathcal{K}}
\providecommand{\cL}{\mathcal{L}}
\providecommand{\cM}{\mathcal{M}}
\providecommand{\cN}{\mathcal{N}}
\providecommand{\cO}{\mathcal{O}}
\providecommand{\cP}{\mathcal{P}}
\providecommand{\cQ}{\mathcal{Q}}
\providecommand{\cR}{\mathcal{R}}
\providecommand{\cS}{\mathcal{S}}
\providecommand{\cT}{\mathcal{T}}
\providecommand{\cU}{\mathcal{U}}
\providecommand{\cV}{\mathcal{V}}
\providecommand{\cX}{\mathcal{X}}
\providecommand{\cY}{\mathcal{Y}}
\providecommand{\cW}{\mathcal{W}}
\providecommand{\cZ}{\mathcal{Z}}

% textstyle math environment.
\newenvironment{talign}
{\let\displaystyle\textstyle\align}
{\endalign}
\newenvironment{talign*}
{\let\displaystyle\textstyle\csname align*\endcsname}
{\endalign}

==> journal/main.tex <==
\begin{abstract}
Gradient tracking (GT) is an algorithm designed for solving decentralized optimization problems over a network (such as training a machine learning model). 
A key feature of GT is a tracking mechanism that allows to overcome data heterogeneity between nodes. 

We develop a novel decentralized tracking mechanism, $K$-GT, that enables communication-efficient local updates in GT while inheriting the data-independence property of GT. 
We prove a convergence rate for $K$-GT on smooth non-convex functions and prove that it reduces the communication overhead asymptotically by a linear factor $K$, where $K$ denotes the number of local steps.
We illustrate the robustness and effectiveness of this heterogeneity correction on convex and non-convex benchmark problems and on a non-convex neural network training task with the MNIST dataset.

%Decentralized machine learning offers better scalability than centralized systems, as the algorithms can benefit from the parallel processing power of many devices, and better data protection, as the training never leaves the device on which it is stored.
%Local update methods enable communication-efficient training with decentralized SGD (D\nobreakdash-SGD). However, the training efficiency and quality of D\nobreakdash-SGD is severely compromised for non-iid datasets.
%Gradient tracking (GT) addresses the problem of data heterogeneity, but at the cost of higher communication cost per iteration.\\
 %In this paper, we develop a novel decentralized tracking mechanism that enables communication-efficient local updates in GT while inheriting its data-independence properties.
%	We prove that the resulting algorithm, $K$-GT, with $K$
%	local updates requires only $\cO(\frac{1}{nK\epsilon^2})$
%	rounds of communications on $n$ devices to converge to an $\epsilon$-approximate stationary point, reducing the communication rounds by a factor of $K$ over the GT baseline.
%    local steps requires $K$ times fewer rounds of communication
%     enjoys linear speedup in the number of parallel devices and gradient evaluations, and converges in  $K$
	%enjoys the convergence rate
	%after $T$ rounds consisting of $K$ local steps each on $n$ devices. Compared to GT, XXX needs $\sqrt{K}$ less rounds of communication to converge to the same accuracy.
	%$\cO(\frac{\sigma}{\sqrt{nT}})$ for GT to
	%We empirically evaluate $K$-GT on image classification tasks (i.e, CIFAR-10 with ResNet) and justify its robustness against data heterogeneity while saving an order of magnitude on communication costs over strong baselines. \looseness=-1
%	Large-scale machine learning (ML) applications benefit from decentralized training, where every device in the system only needs to communicate with a few number of neighbor-devices.
%	Typically, heterogeneous data is presented on each device, hindering the quality of decentralized optimization.
%	Existing methods such as stochastic Gradient Tracking (GT), though can tackle this data heterogeneity issue, are yet sensitive to communication cost. \\
%	In this paper, we propose a new communication-efficient decentralized stochastic algorithm, a.k.a. $K$\nobreakdash-GT, that is robust to heterogeneous data and less vulnerable to communication cost.
	% allows for local steps, called $K$\nobreakdash-GT.
%	Our algorithm is a non-trivial extension of the GT algorithm, and its convergence is independent of data-heterogeneity for any topology.
%	Moreover, our $K$\nobreakdash-GT improves the convergence rate from $\cO(\frac{\sigma}{\sqrt{nT}})$ for GT to $\cO(\frac{\sigma}{\sqrt{nKT}})$ by using $K$ local steps.
%	We empirically evaluate $K$\nobreakdash-GT on image classification task (i.e, CIFAR-10 with ResNet) and justify its robustness against data heterogeneity while saving an order of magnitude on communication costs over strong baselines. \looseness=-1
	% by more efficiently using the local steps.
\end{abstract}

\section{Introduction}
 %\yue{introducing the optimization problem with concise descriptions.}Distributed optimization~\citep{Dekel2012:minibatch, federated-opt,  mcmahan2017communication, local-sgd1, Yu2018parallel} is an important paradigm, due to the massive rise up of many applications scenarios, e.g. edge computing, federated learning and modern large-scale machine learning (ML) systems, in which every step of measurement and optimization are conducted locally on edge devices (clients) without exchanging their local datasets.

%In classical optimization problems, one optimizes just one function, while in the problem of %SEB: not very specific, was is classic?

We consider distributed optimization problems,
where the objective function $f(\xx)$ on model $\xx \in \R^d$ is defined as the average of $n$ different components $\{f_1(\xx), ..., f_n(\xx)\}$, i.e., $$f(\xx)=\frac{1}{n}\sum_{i=1}^nf_i(\xx).$$  In distributed applications, different contributors (or `clients') take part in the training.
Such clients can be, for example, mobile edge devices, or computing nodes. Typically, each component $f_i(\xx)$ is only available to a single client (for instance, when $f_i(\xx)$ is defined over the training data available only locally  on the client). This makes distributed optimization problems more difficult to solve than centralized problems.

%\yue{the introduction of the usage and importance of communication.}
Besides convergence rate in terms of iterations, communication efficiency is one of the most important metrics in distributed algorithm design. For illustration we consider the calculation of a gradient of the global function, $\nabla f(\xx) = \frac{1}{n}\sum_i\nabla f_i(\xx)$, that forms be basis for general first-order methods. Since each client only has the ability to evaluate the local gradient $\nabla f_i(\xx)$, it is further necessary to calculate the average of these local gradients.
% the average of those local gradients still yields the desired gradient of the global loss for general first-order methods. 
Centralized algorithms~\citep{fedcomm, mcmahan2017communication} realize such global aggregation by a central controller, e.g., with a parameter sever~\citep{ps}. However, this approach requires all clients to communicate with the central server simultaneously, resulting in a communication bottleneck at this hot point and a slowdown in clock time. Instead of the exact averaging, decentralized algorithms~\citep{tsitsiklis1984problems, de>cen,KoloskovaLSJ19decentralized} require only partial communication through gossip averaging and reduce communication overhead by allowing a node to communicate with fewer nodes, e.g., only its neighbors, thus avoiding having the busiest point.  How nodes are connected between each other makes up the network topology.\looseness=-1

%Decentralized  convergence is still comparable to the centralized~\citep{de>cen}. %SEB: why is then this paper needed? need to be more precise (or removed for now)

One of the most challenging aspects in decentralized optimization is data-heterogeneity, that is when the training data is not identically and independently (non-\iid) distributed across the nodes.
Such non-\iid distributions often arise in practical applications, since, for example, training data originating from cell phones, sensors, or hospitals can have regional differences~\cite{client-sampling}.
%Heterogeneous data causes optimization difficulties,
In this case, the local empirical losses on each client are different.
This can slow down the convergence~\citep{dsgd, unified-dsgd} or even yield local overfitting (often termed \emph{client\nobreakdash-drift}) as the clients
may drift away from the global optimum in the course of the optimization process~\citep{scaffold, non-iid-benchmark, noniid, unified-dsgd}.
% This phenomena has been
% in theoretical analysis~\citep{unified-dsgd}

%% Heterogeneous data results in diverse optimization objectives on each client,
%which hampers the global convergence in theoretical analysis~\citep{unified-dsgd}, as well as 'client\nobreakdash-drift' in empirical analysis~\citep{scaffold, non-iid-benchmark, noniid}. Client\nobreakdash-drift is the model quality loss when the model drifts from the global optimum.
There are several decentralized algorithms that have been shown to mitigate heterogeneity. However, most of them are proven to converge for only strongly convex functions~\citep{extra_convex,primal-dual,diging,gt-svrg,network-svrg}, or are proven for smooth non-convex functions but have a strict constraint on network topologies~\citep[such as e.g.][]{d2_nonconvex}.  %Deterministic algorithms EXTRA~ and primal-dual methods~\citep{primal-dual} depends only on data heterogeneity on the initial point and achieve linear convergence, but only for  strongly convex functions. DIGing~\citep{diging} based on deteministic gradient tracking supports time-varying topologies for convex functions. There also exists stochastic algorithms proven to work better on heterogeneous clients. GT-SVRG~\citep{gt-svrg} and Network-SVRG~\citep{network-svrg}, based on variance-reduction framework~\citep{svrg, saga} achieve linear convergence only in the strongly convex cases. $D^2$~\citep{d2_nonconvex} asymptotically converges on non-convex functions, but has a constraint on network topologies. Stochastic gradient tracking~\citep{gt, gt-nonconvex, koloskova2021improved} works on arbitrary network for non-convex functions
Stochastic gradient tracking~(GT)~\citep{Lorenzo2016GT-first-paper, diging, gt, gt-nonconvex, koloskova2021improved} algorithms have been proposed to address data-heterogeneity for arbitrary networks for smooth non-convex functions. Its convergence rate only depends on the data heterogeneity at the initial point, which can be completely removed with proper initialization.
However, the clients are required to communicate with all their neighbors in the network after every single model update.
%when using these algorithms, the clients need to communicate with all their neighbors after every  model update.
These methods are still therefore associated with high communication overheads.

% and $D^2$~\citep{d2_nonconvex} are the modification
%In contrast, there exist algorithms that correct for the data-heterogeneity in the context of decentralized stochastic optimization. Gradient tracking~(GT)~\citep{Lorenzo2016GT-first-paper, diging, gt, gt-nonconvex} and $D^2$~\citep{d2_nonconvex} are the modification of Decentralized stochastic gradient descent~(D\nobreakdash-SGD), and they are designed for fixed typologies on non-convex functions. However, they all need to communicate for every step of model update thus having heavy communication overhead.
In order to further reduce communication overhead within distributed training, various engineering techniques have been proposed, such as using large batch~\citep{large-mini-batch, large-mini-batch-2, largebatch}, model/gradient compression~\citep{dsgd-compression} or asynchronized communication~\citep{async-dsgd}. In this work, we focus on local updates to reduce communication frequency, which is often efficient in practice but remains challenging in the theoretical analysis~\citep{mcmahan2017communication, local-sgd1, local-sgd2,fedcomm}. However, performing a large number of local steps can
\emph{exacerbate} the client\nobreakdash-drift.
The resulting optimization difficulties can negate the communication savings~\citep{scaffold, unified-dsgd}. %Local SGD has been quite systematically studied given the tight analysis from identical~\citep{federated-opt}, limited heterogeneous~\citep{local-sgd1, local-sgd2} to heterogeneous functions~\citep{scaffold, unified-dsgd}. 
The analysis of incorporating local steps while heterogeneity independence in the decentralized optimization is still seldom investigated. 

%In order to further reduce communication overhead within distributed training, recent works proposed to perform several local update steps on the clients between each communication round~\citep{mcmahan2017communication, local-sgd1, local-sgd2}.
%This allows to reduce the communication overhead.
%It's possible to reduce communication overhead by periodical communication. It enables clients to update model locally for steps before they communicate~\citep{mcmahan2017communication, local-sgd1, local-sgd2}.
%However, performing a large number of local steps can
%\emph{exacerbate} the client\nobreakdash-drift.
%The resulting optimization difficulties can negate the communication savings, as more iterations are needed.

% lead to ‘over\nobreakdash-fitting’ to the heterogeneous local data, which exacerbates the client\nobreakdash-drift. %\yue{perhaps local steps would further enlarge the impact of heterogeneity.}

%SEB: I do not get this paragraph, there is no evidence presented here
%
%Intuitively, we consider GT on time-varying topology which alternates between identity matrix~(no communication, local steps) and others~(communication). We prove this 'Periodical GT'~(Alg.~\ref{algo: tv_gt1}) still converges independent of heterogeneity but asymptotically need only $\cO(\frac{1}{nK\epsilon^2})$ communication rounds with $K$ local steps on $n$ devices to approximate $\epsilon$-approximate stationary point, compared to $\cO(\frac{1}{n\epsilon^2})$ for GT baseline. However, Periodical GT seldom works well in practice~(in Figure~\ref{fig: simulation},~\ref{fig: local_steps}), suffering from severe stochastic noise. %We prove that iHowever, it currently doesn't have any theoretical guarantee to show that its convergence rate is independent of heterogeneity. Besides, it suffers from severe client\nobreakdash-drift on DNN models~(shown in Figure~\ref{fig: local_steps}).

Integrating local updates into GT is non-trivial.
For instance, simply skipping communication rounds in GT (and thereby performing a number of local updates in-between)
does not work well in practice\footnote{We evaluate this variant (termed \emph{periodical GT}) below in Section~\ref{sec:experiments}, see e.g.\ %Figure~\ref{fig: simulation_convex} and 
Figure \ref{fig: mnist}.}. % SEB: I removed the first link, as there it works well
%
A concurrent work LU\nobreakdash-GT\citep{lu-gt} analyzed the performance of GT periodically skipping the communication but only in the deterministic setting.\footnote{This concurrent work was independently developed while we were finalizing this manuscript. We will add a more detailed comparison to the next version of this manuscript.}

As a solution, we carefully design a novel tracking mechanism that enables to combine GT with local steps.\footnote{Partial results of this paper where previously presented in YL's master thesis~\citep{thesis}}
%Our mechanism, based on a variance reduction technique,
The resulting algorithm---$K$-GT, where $K$ denotes the number of local steps---is a novel decentralized method that provides communication-efficient tracking with local updates.
We prove that the convergence of $K$-GT depends only on the data heterogeneity at the starting point and that this weak data dependence can be completely circumvented with an additional round of global communication.
As long as $K$\nobreakdash-GT uses the same initialization as GT,  $K$\nobreakdash-GT inherits the heterogeneity independence property of GT.
%sum tracking by variance-reduction-like technique
%As a solution, we propose a novel decentralized method that enables communication-efficient tracking with local updates while inheriting its heterogeneity-independence properties. Instead of modifying topology, $K$\nobreakdash-GT is a non-trivial extension of gradient tracking to gradient sum tracking by variance-reduction-like technique.
We prove that $K$\nobreakdash-GT~(Algorithm~\ref{algo: k-gt}) achieves asymptotically linear speed-up in terms of communication round w.r.t.\ local steps $K$ and number of clients $n$, and that it converges in $\cO\big(\frac{\sigma^2}{nK\epsilon^2}\big)$ rounds to an $\epsilon$-approximate stationary point.
The number of communication rounds is asymptotically reduced by a factor of $K$ compared to GT.
We further show that the convergence rate (including higher order terms) does not depend on
the data-heterogenity if with proper initialization, opposed as e.g.\ for decentralized stochastic gradient descent~(D\nobreakdash-SGD) without tracking. %Besides, we also show that in implementations, $K$\nobreakdash-GT is much more robust against data-heterogeneity with arbitrary initialization.
\looseness=-1
%Compared to the GT baseline, $\cO\big(\frac{1}{n\epsilon^2}\big)$
%SEB: move to contributions
%We empirically justify the methods robustness across heterogenous setting while it can always recover the best generalization performance even with large number of local steps~(in Figure~\ref{fig: local_steps}).

%SEB: move this discussion much later
%Finally, we observe $K$\nobreakdash-GT is possibly equivalent to the centralized algorithm, SCAFFOLD~\citep{scaffold} when network topology is a complete graph.
The outline of this paper is as follows:\ In Section 2, we give the precise formulation of the distributed optimization problem setting.  In Section 3, we introduce the algorithm design of $K$-GT and demonstrate how it helps to correct for heterogeneity. Here, our main result state its convergence rate, see Theorem~\ref{thm: k-gt}. In Section 4, we generalize the gradient tracking framework and discuss about the drawbacks of other GT alternatives that could also be stemmed from the same framework. We in addition contribute their convergence results and give a comparison to show that $K$-GT is the most communication efficiency theorectically. In Section 5, we compare the GT-variants with baseline D-SGD with numerical examples in detail.
\paragraph*{Contributions.} We summarize our main results below.
\begin{itemize}[leftmargin=12pt,nosep,itemsep=1pt]
 \item We develop a novel gradient tracking algorithm for distributed optimization and analyze its convergence properties. We prove that $K$\nobreakdash-GT enjoys heterogeneity-independent complexity estimates (with proper initialization)
  and prove that it converges asymptotically in  $\cO\big(\frac{\sigma^2}{nK\epsilon^2}\big)$ rounds, where $n$ denotes client number, $K$ the number of local steps, $\sigma^2$ the stochastic noise level and $\epsilon$ the accuracy. This improves by a factor of $K$ over the GT baseline.
% 	\item On the theory side, We are the first to extent the analysis of the GT algorithm to the GT with $K$ local steps, and to show that both Periodical GT and $K$\nobreakdash-GT asymptotically converge at the rate of $\cO(\frac{\sigma}{\sqrt{nKT}})$ for non-convex functions in the presence of stochastic noise given $T$ communication rounds and both inherit heterogeneity-independence property from GT baseline.   %The use of $K$ local steps enables Periodical GT and $K$\nobreakdash-GT to communicate once every $K$ iterates thus greatly decreasing the communication frequency compared to standard GT. And comparing to other decentralized stochastic algorithms with local steps,
 \item We provide additional theoretical insights, by studying
 (i) the convergence of the na\"ive local extension of GT, \emph{periodic GT}, explaining that it performs worse than $K$-GT when the stochastic noise is large, and
 (ii) a computationally inefficient variant, \emph{large-batch GT} that matches the iteration, but not the computation complexity of $K$-GT.
%
%	\item In the non-asymptotic regime (of importance in practice), we show that Periodical GT suffers more from stochastic noise than $K$\nobreakdash-GT. We improve the convergence of Periodical GT by inserting full-batch gradient and verify it in numerical experiments.
	\item We empirically verify the theoretical results on strongly convex and non-convex functions and explain the impact of noise, local steps and data-heterogeneity on the convergence. %And we also evaluate the performance of $K$-GT on image classification tasks with deep neural network (DNN), i.e, ResNet~\cite{resnet} with CIFAR-10~\cite{cifar10}, and 
$K$-GT is robust against the data-heterogeneity while improving the communication efficiency and  improves generalization performance over baseline algorithms.
\end{itemize}


%\paragraph*{Related work.}
%SEB: Decentralized stochastic gradient descent~(D\nobreakdash-SGD)
%
%Decentralized optimization can be traced back to~\cite{tsitsiklis1984problems}. For different application, various techniques have been purposed. Push-sum algorithms are modelled based on Markov chains and considering asymmetric communication or the symmetric time-varying gossip protocol for averaging over arbitrary graphs,~\citep{boyd2006randomized}, which we follow in this work. In addition, there are various algorithms that are specifically tailored to the problem's structure, for instance the alternating direction method of multipliers~\citep{admm}, dual averaging~\citep{dual-average1}, and primal-dual methods~\citep{primal-dual}.

%Distributed gradient-based methods  suffer from a `client\nobreakdash-drift'~\citep{client-drift, scaffold} when clients have heterogeneous data. The discrepancy among the local loss functions leads to a drift on each client towards their local minima---potentially far away from the global minimum. Besides, the data-heterogeneity also slows down the convergence~\citep{dsgd, unified-dsgd}.

%In contrast, there are decentralized algorithms proven to mitigate heterogeneity.  Deterministic algorithms EXTRA~\citep{extra_convex} and primal-dual methods~\citep{primal-dual} depends only on data heterogeneity on the initial point and achieve linear convergence, but only for  strongly convex functions. DIGing~\citep{diging} based on deteministic gradient tracking supports time-varying topologies for convex functions. There also exists stochastic algorithms proven to work better on heterogeneous clients. GT-SVRG~\citep{gt-svrg} and Network-SVRG~\citep{network-svrg}, based on variance-reduction framework~\citep{svrg, saga} achieve linear convergence only in the strongly convex cases. $D^2$~\citep{d2_nonconvex} asymptotically converges on non-convex functions, but has a constraint on network topologies. Stochastic gradient tracking~\citep{gt, gt-nonconvex, koloskova2021improved} works on arbitrary network for non-convex functions. However, this algorithm requires communication for every step of model update which results in rather high communication cost.

% \ak{GT with time-varying topology is called DIGing and there been some literature about that. Good to mention and compare (not for convex ? bad convergence rate ? ). }
% \ak{There are also primal-dual algorithm. Mention that EXTRA is only for convex, non-stochastic (?). }

%For reducing communication cost, various techniques have been proposed, such as using large batch~\citep{large-mini-batch, large-mini-batch-2, largebatch}, model/gradient compression~\citep{dsgd-compression} or asynchronized communication~\citep{async-dsgd}. But in this work, we focus on local updates to reduce communication frequency, which is often efficient in practice but remains challenging in the theoretical analysis~\citep{fedcomm}. Local SGD has been quite systematically studied given the tight analysis from identical~\citep{federated-opt}, limited heterogeneous~\citep{local-sgd1, local-sgd2} to heterogeneous functions~\citep{scaffold, unified-dsgd}. But the analysis of incorporating local training while heterogeneity independence in the decentralized training is still seldom investigated.
%\begin{comment}
\begin{table}[tb]
\caption{A comparison under different working conditions. $\Delta \leq n$ denotes the maximum degree of the communication graph. $K$-GT is the first fully-decentralized tracking algorithm with local steps.}% \iseb{I think $\max(n,\Delta)=n$ in all cases?; and for the last column should it be reversed? (maybe a different column title?)}
\renewcommand{\arraystretch}{1.1}
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{lccc}
			\toprule[1pt]
			\multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{c}{\textbf{Settings}}\\\cline{2-4}
			   &  \makecell[c]{Communication cost at the busiest point}& Local steps & \makecell[c]{heterogeneity-robustness\textsuperscript{a}} \\ \midrule[0.8pt]
			  \makecell[l]{SCAFFOLD~\citep{scaffold}} & $\cO(n)$& \cmark & \cmark\\\hline
			  \makecell[l]{GOSSIP\nobreakdash-PGA~\citep{gossip-pga}} & \multirow{5}{*}{$\cO(\Delta)$} & \cmark & \xmark \\\cline{1-1}\cline{3-4}
			\makecell[l]{D\nobreakdash-SGD~\citep{unified-dsgd}} &  & \cmark & \xmark \\\cline{1-1}\cline{3-4}
			\makecell[l]{GT~\citep{diging}} &  & \xmark &\cmark \\\cline{1-1}\cline{3-4}
			\makecell[l]{$D^2$~\citep{d2_nonconvex}} &  & \xmark &\cmark \\\cline{1-1}\cline{3-4}
			\makecell[l]{$K$\nobreakdash-GT {\textbf{[ours]}} }  &  & \cmark & \cmark \\
			\bottomrule[1pt]
		\end{tabular}}
\tabnote{\textsuperscript{a}The data heterogeneity does not impact the worst-case convergence rate (but might require special initialization).}		
	\label{tab: comparison}
\end{table}
%\end{comment}
%\footnotetext[1]{Mixture communication means it needs to perform both centralized and decentralized communication.}
%\vspace{-6mm}
\section{Problem setting}
%\vspace{-1mm}
%We introduce the decentralized SCAFFOLD algorithm in this section.
We introduce the notation and setup in this section.
%\vspace{-9mm}
\subsection{Decentralized Optimization Problem}
We consider the optimization problems as the summation from $n$-client loss functions, \begin{equation}
	\underset{\xx \in \mathbb{R}^d}{\mbox{min}} f(\xx):=\frac{1}{n}\sum_{i=1}^n \left[f_i(x) := \mathbb{E}_{\xi_i\sim \cD_i}F_i(\xx;\xi_i) \right]\,,
	\label{eq: global function}
\end{equation}
where $n$ denotes the number of clients within the system, $\xi_i$ is a random sample from $\cD_i$ and $\cD_i$ denotes the local distribution only available on node $i\in[n]$. $\cD_i$ could be arbitrary and different among clients considering the applications. This setup  models both empirical risk minimization and the online optimization setting. 

In this work, we consider general smooth non-convex functions and bounded stochastic noise.
\begin{assumption}[Smoothness]\label{ass: smooth}Each function $f_i(x):\mathbb{R}^d\rightarrow\mathbb{R},\ \forall i\in[n]$ is differentiable and there exists a constant $L>0$ such that for each $\xx,\ \yy\in\mathbb{R}^d$, 
\begin{equation}\nonumber
	f_i(\yy)\leq f_i(\xx) + \nabla f_i(\xx)^T(\yy-\xx) + \frac{L}{2}||\xx-\yy||_2^2 \,.
\end{equation}%\begin{equation}\nonumber||\nabla f_i(\xx)-\nabla f_i(\yy)||\leq L||\xx-\yy||\end{equation}
\label{ass:l}
\end{assumption}
\vspace{-5mm}
\begin{assumption}[Bounded variance]Each client variance is uniformly bounded, 
	\begin{equation}\nonumber
		\begin{aligned}
			  \forall i\in[n],\  \forall \xx \in \R^d,\ \mathbb{E}_{\xi \sim \cD_i}||\nabla F_i(\xx; \xi)-\nabla f_i(\xx)||_2^2\leq \sigma^2 \,.
		\end{aligned}
	\end{equation}
	\label{ass:noise}
\end{assumption}
\vspace{-10mm}

\subsection{Communication graph}The training is implemented over a decentralized network, and its topology is modelled as an undirected graph: $(\cV, \cE)$, where $\cV:=\{ 1, 2, \ldots, n \}$ is the node set and $\cE \subseteq \cV \times \cV$ is the edge set. Node~(or client) represents a computing node, and clients communicate only along the edges $e\in\cE$. We denote the adjacency matrix $\mW\in\mathbb{R}^{n\times n}$, where $w_{ij}=0$ means node $i$ and $j$ are not connected, i.e., $e_{ij}=(i,j)\notin\cE$.
\begin{assumption}[Mixing rate] Given the symmetric and doubly stochastic mixing matrix $\mW\in\mathbb{R}^{n\times n}$ of nonnegative real numbers, i.e., $\forall i,j\in[n],\ w_{ij}\geq 0$, $\textstyle \sum_{i=1}^n w_{ij} = \textstyle  \sum_{j=1}^n w_{ij} = 1,$ the consensus distance decreases linearly after averaging step, i.e. there exists a $1\geq p>0$ such that $$||\mX\mW - \bar\mX||_F^2\leq (1-p)||\mX - \bar\mX||_F^2,\ \forall \mX \in \R^{d \times n}\,.$$
\label{ass:p}
\end{assumption}\vspace{-5mm}
Note that if the commonly used network parameter $\rho:=||\mW-\frac{\unit_n\unit_n^T}{n}||$~\cite{gossip-pga} is strictly less than 1, then $1\geq p>0$ \citep[see e.g.][]{unified-dsgd, koloskova2021improved}.
The mixing rate describes the connectivity of the network. The larger value of $p$ means the communication graph is better connected. $p=1$ for a complete graph $\mW = \tfrac{1}{n}\unit\unit^T$, and $p=0$ for a disconnected graph $\mW = \mI_n$.

%\vspace{-2mm}

\subsection{Data heterogeneity and correction}
When the local distributions $\{\cD_i\}$ are identical on each client, the local functions $\{f_i(\xx)\}$ are identical to each other, i.e., $f_i(\xx)\equiv f(\xx)$. Otherwise, heterogeneous local distributions result in heterogeneous local functions. And heterogeneity is usually measured by the discrepancy between local gradients $\{\nabla f_i(\xx)\}$ and global gradient $\nabla f(\xx)$~\cite{scaffold,unified-dsgd} as follows.
\begin{assumption}[Data-heterogeneity]\label{ass: noniid} There exists constants $\zeta^2>0$ and $B\geq 1$ such that  \begin{equation}\nonumber\forall \xx\in\mathbb{R}^d,\ \frac{1}{n} \sum_{i=1}^n ||\nabla f_i(\xx)||^2\leq \bar\zeta^2+B^2||\nabla f(\xx)||^2\,,\end{equation} where both $\bar\zeta^2$ and $B^2$ represent the degree of heterogeneity within the system.
\label{ass:zeta}
\end{assumption}
The baseline Decentralized SGD~(D\nobreakdash-SGD) uses na\"{i}ve gradient w.r.t local model, the convergence of which inevitably are influenced by both $\bar\zeta^2$ and $B$~\citep{dsgd}.
\subsubsection{Notations}
Gradient tracking algorithm mainly manipulates between two variables, model iterate $\xx\in\mathbb{R}^d$ and tracking variable $\zz\in\mathbb{R}^d$. More precisely, we denote vector $\yy\in\{\xx,\ \zz\}$ as $\yy_i^{(t)+k}$ on node $i$ in local step $k$ at communication round ${t}$, and denote its average by $\bar\yy = \frac{1}{n}\sum_i\yy_i$.
%$\xx_i^{(t)+k}\in\mathbb{R}^d$
% \ak{Shorten below by describing it for an arbitrary sequence of vectors, say $\{\aa_i\}$ that could be either $\xx_i$ or $\zz_i$. }

% \ak{Above was $Y$, and now here $Z$, unify. }
The collection of vectors $\yy_i$ for all $i\in[n]$ in matrix form is denoted by a capital letter with columns $\yy_i$, i.e., $$\mY = \begin{bmatrix}\yy_1, \ldots, \yy_n\end{bmatrix}\in\mathbb{R}^{d\times n},\quad \bar\mY = \begin{bmatrix}\bar\yy, \ldots,  \bar\yy\end{bmatrix}= \tfrac{1}{n}  \mY\unit_n\unit_n^T\in\mathbb{R}^{d\times n}\,.$$
Also, we extend this matrix definition to both gradient and stochastic gradient of (\ref{eq: global function}) w.r.t model $\mX$ on sample $\xi=[\xi_1,\ \ldots,\ \xi_n]$, where $\xi_i\sim \cD_i,$
\begin{equation}\nonumber
	\begin{aligned}
		\nabla F(\mX;\xi) &=\begin{bmatrix}\nabla F_1(\xx_1;\xi_1),\ldots,\nabla F_n(\xx_n;\xi_n)\end{bmatrix}\in\mathbb{R}^{d\times n},	\\
		\nabla f(\mX)&=\mathbb{E}_{(\xi_1, \ldots, \xi_n)}\nabla F(\mX;\xi)
		=\begin{bmatrix}\nabla f_1(\xx_1), \ldots, \nabla f_n(\xx_n)\end{bmatrix}\in\mathbb{R}^{d\times n}\,.
	\end{aligned}
\end{equation}
%\vspace{-7mm}
\subsubsection{Gradient tracking}
Gradient tracking algorithm~(GT)~\cite{gt} is defined by the following update equations:
\begin{equation}\label{eq: dsgt}
	\begin{aligned}
		\mX^{(t+1)} & = (\mX^{(t)}-\eta \mZ^{(t)})\mW                               \\
		\mZ^{(t+1)} & = \mZ^{(t)}\mW +\mG^{(t+1)} -\mG^{(t)},
	\end{aligned}
\end{equation}
in matrix format. Here $\mG^{(t)} = \nabla F(\mX^{(t)}; \xi^{(t)})$ and $\eta>0$ denotes the stepsize. 

When data is heterogeneous among different nodes, $\{\nabla F_i(\xx;\xi_i),\ \forall i\}$ are different. But GT uses bias-correction to compensate heterogeneous gradient at each node. This correction is governed by the tracking variable $\mZ$ that replaces the na\"{i}ve gradient: \begin{equation}\label{eq: dsgt_corr}\mZ^{(t+1)} = \nabla F(\mX^{(t+1)}; \xi^{(t+1)}) + \underbrace{ \mZ^{(t)}\mW  -\mG^{(t)}}_{\text{correction}}\end{equation} Since the update (\ref{eq: dsgt}) simultaneously updates both the model $\mX$ and the tracking variable $\mZ$, there is no need to take extra consideration on the heterogeneous local gradient. GT is proven to converge regardless of data heterogeneity~\citep{gt}.


\section{K-GT: Gradient Sum Tracking algorithm}
In this section, we present our new decentralized stochastic algorithm $K$\nobreakdash-GT with its convergence analysis for general non-convex functions.
%, and discuss its superiority by comparing to other GT-like alternatives that have the same communication pattern.

%\subsection{DSGT with local steps}
%However, DSGT must sent out models to neighbors every iterate, and it may hurt the network bandwidth when model is large or network is busy.  We consider instead of communicating every iterate but once every $K$ steps. Then it literally could achieve the acceleration in terms of communication rounds propotional to $\frac{1}{K}$.

%$\mX^{mK}$, $\forall m\in\mathbb{N}^{+}$ is updated by gossip averaging every $K$ step. Literally, similar to that in case with single step, the tracking variable $\mZ^{mK}$ is updated every $K$ steps as well.  Then consider the following generalized communication scheme for DSGT with local steps between consecutive communication.

%where $K$ is the number of local steps.
%\begin{proposition} When $K=1$, DSGT with local steps is equivalent to DSGT.
%\end{proposition}
%Apparently, the tracking variable $\mZ^{mK}$ in (\ref{eq: dsgt_local_steps}), also the update from $\mX^{mK}$ to $\mX^{(m+1)K}$ is the result after $K$ sequential steps, $\mX^{mK}\rightarrow\mX^{mK+1}\rightarrow\ldots\rightarrow\mX^{(m+1)K-1}\rightarrow\mX^{(m+1)K}$. Unlike in the single step case (\ref{eq: dsgt}), tracking variable only calcualtes on the progress between one step from $\mX^t$ to $\mX^{t+1}$, the tracking $\mZ^{mK}$ is supposed to depend on accumulated progress after $K$ steps.

%Consider following possible extensions within this framework to improve the communication efficiency of GT.
\vspace{-3mm}
\subsection{Algorithm}
In the $K$-GT algorithm we allow each client to perform $K \geq 1$ local steps between each communication round. To compensate to the data-heterogeneity, we use a similar correction as in  (\ref{eq: dsgt_corr}) on top of the stochastic gradient. We denote the correction as $\cc_i$ on node $i$. Then each node repeats the following updating rule, $i\in[n]$:
\begin{enumerate}
	\item Compute a local stochastic gradient $\nabla F_i(\xx_i; \xi_i)$ by sampling $\xi_i$ from distribution $\cD_i$;
	\item Update the local model $\xx_i^{(t)+k+1}= \xx_i^{(t)+k} - \eta_c \bigl(\nabla F_i(\xx_i^{(t)+k}; \xi_i^{(t)+k}) + \cc_i^{(t)}\bigr)$ using the stochastic gradients at $(t)+k$-th iteration and correction $\cc_i^{(t)}$ in $t$-th communication;
	\item Repeat step (1)-(2) $K$ times, then obtain the tracking throughout local steps, $\zz_i^{(t)}  = \frac{1}{K\eta_c} \bigl(\xx_i^{(t)} - \xx_i^{(t)+K}\bigr)$. Exchange $\{\xx_i, \cc_i\}$ with neighbors: (in matrix format):\begin{equation}\label{eq: k-gt}
	\begin{aligned}
		\mX^{(t+1)} & = \Big(\mX^{(t)} - \eta_s(\mX^{(t)}-\mX^{(t)+K})\Big)\mW	\, ,\\
		\mC^{(t+1)} & = \mC^{(t)} + \mZ^{(t)}(\mW -\mI) \,.	\\
	\end{aligned}
\end{equation}
\end{enumerate}
The complete algorithm is summarized in Algorithm~\ref{algo: k-gt}.
%We develop a new GT-like algorithm to solve the optimization problem~(\ref{eq: global function}). $K$\nobreakdash-GT needs only periodical communication after every $K$ local steps thus reducing communication frequency.
\vspace{-2mm}
\begin{restatable}[Gradient Sum Tracking]{proposition}{localgt}
\label{cor: local_gt}
Define $\mZ^{(t)} = \frac{1}{K\eta_c}\Big(\mX^{(t)} - \mX^{(t)+K}\Big)$ as the tracking variable during communication round~$t$. The update rule for both models $\mX^{(t)}$ and tracking variables $\mZ^{(t)}$ at communication in $K$\nobreakdash-GT can be rewritten as ($\eta=\eta_s\eta_c$):
\begin{equation}
	\begin{aligned}
		\mX^{(t+1)} & = \Big(\mX^{(t)}-K\eta\mZ^{(t)}\Big)\mW \,, \\
		\mZ^{(t+1)} & = \mZ^{(t+1)}\mW + \mG^{(t+1)} - \mG^{(t)}\,,
	\end{aligned}
	\label{eq: local_gt}
\end{equation}
where $\mG^{(t)} = \frac{1}{K} \sum_{k}\nabla F(\mX^{(t)+k};\xi^{(t)+k})$ denotes the mean update over the local steps.% and $\eta=\eta_s\eta_c$. %The tracking is extented from gradient in GT to gradient sum over $K$ local steps in $K$\nobreakdash-GT.
\end{restatable}

The detailed proof is included in Appendix~\ref{ap: gt}.
\begin{remark}\label{remark: equivalence}
If $K=1$ in~(\ref{eq: local_gt}), $K$\nobreakdash-GT is equivalent to Gradient Tracking~\citep{gt} with $\eta=\eta_s\eta_c$.
\end{remark}
\paragraph*{$K$-GT essentially runs SGD if communication is the most sufficient.} To understand the intuition behind $K$-GT, let us consider the global average $\bar\mX$ at each iterate, which gets updated just like the standard stochastic gradient descent:
\begin{equation}	\nonumber
	\begin{aligned}	
		\bar\mX^{(t)+k+1} &= \Big(\mX^{(t)+k} - \eta_c(\nabla F(\mX^{(t)+k}; \xi^{(t)+k}) + \mC^{(t)})\Big)\tfrac{\unit\unit^T}{n}	\\
		& = \bar\mX^{(t)} - \eta_c\Big(\overline{\nabla F(\mX^{(t)+k}; \xi^{(t)+k})} + \bar\mC^{(t)}\Big) \,.
	\end{aligned}
\end{equation}
If initialized to be $\mC^{(0)} = \nabla F(\mX^{(0)}; \xi^{(0)})\bigl(\frac{\unit\unit^T}{n} - \mI\bigr)$, the average of correction satisfies 
\begin{equation}\nonumber
	\begin{aligned}
		\bar\mC^{(t+1)} & = \bar\mC^{(t)}+ \mZ^{(t)}(\mW - \mI)\tfrac{\unit\unit^T}{n} = \bar\mC^{(t)} \,,	\\
		\bar\mC^{(0)} & = \nabla F(\mX^{(0)}; \xi^{(0)})\left(\tfrac{\unit\unit^T}{n} - \mI\right)\frac{\unit\unit^T}{n}	 \equiv \zero \,.
	\end{aligned}
\end{equation}
Then the average of model iterate satisfies $$\bar\mX^{(t)+k+1} = \bar\mX^{(t)} - \eta_c\overline{\nabla F(\mX^{(t)+k}; \xi^{(t)+k})},$$ which updates model with averaged stochastic gradient. 

\paragraph*{How does this correction improves D-SGD?} We consider applying the similar analysis from~\cite{d2_nonconvex} to illustrate the effectiveness of $K$-GT.
Assume that $\mX^{(t)}$ has achieved an optimum $\mX^{\star} : = \xx^{\star}\unit^T$ with all local models equal to the optimum $\xx^{\star}$. Based on our analysis in appendix~(Lemma~\ref{lemma: correction}), the correction will be equal to $$\cc_i^{\star} :=-\nabla F_i(\xx^{\star}; \xi) + \frac{1}{n}\sum_{j}\nabla F_j(\xx_j^{\star}; \xi)\,.$$ Then the next local update for $K$-GT would be
\begin{equation}\nonumber 
	\begin{aligned}
		\mX^{(t)+1} &= \mX^{\star} -\eta_c(\nabla F(\mX^{\star}; \xi) + \mC^{\star})	\\
		& = \mX^{\star} -\eta_c\nabla F(\mX^{\star}; \xi)\tfrac{\unit\unit^T}{n} \,.
	\end{aligned}
\end{equation}
This illustration shows that for $K$-GT, the convergence when we approach a solution with only local update relies on the magnitude of $\mE||\nabla F(\mX^{\star}; \xi)\frac{\unit\unit^T}{n}||_F^2$, which is bounded by $\cO(\sigma^2)$. 

However, consider the same situation for D-SGD, 
\begin{equation}\nonumber
	\begin{aligned}
		\mX^{(t)+1} &= \mX^{\star} -\eta\nabla F(\mX^{\star}; \xi). 	\end{aligned}
\end{equation}On different nodes, $\nabla F_i(\mX^{\star}; \xi)$ deviates from each other due to data heterogeneity, and the deviation can only be characterized by $\zeta^2$ as suggested in Assumption~\ref{ass: noniid}. Then the upper bound for D-SGD of the same magnitude of convergence when in the neighborhood of solution is $\cO(\sigma^2 + \bar\zeta^2)$~\citep{d2_nonconvex}, which is obviously worse than that for $K$-GT. The additional $\cO(\bar\zeta^2)$ in D-SGD from the data heterogeneity can never be improved if always using the sole stochastic gradient~\citep{dsgd}. %\paragraph*{Local update with correction mitigates the heterogeneity.} %When data heterogeneity among clients, the local SGD $\nabla F_i(\xx; \xi)$ on clients also deviates from each other. 
%We correct $\nabla F_i(\xx; \xi)$ to shift towards the "true" direction. The correction $\cc_i\in\mathbb{R}^{d}$ is supposed to capture the difference between local update on client $i$ and global update if performing centralized averaging.
%\yue{[todo] need more discussion on how mitigation works. And what kind of further interpretation are needed?}

%\begin{equation}\nonumber
%	\begin{aligned}
%		\mX^{(t+1)}& = \bigg(\mX^{(t)} - \eta_s(\mX^{(t)} - \mX^{(t)+K})\bigg)\mW \\
%		\mZ^{(t+1)} & = \bigg(\frac{1}{K}\sum_k\mZ^{(t)+k}\bigg)\mW + \nabla F(\mX^{(t+1)};\xi^{(t+1)}) -  \frac{1}{K}\sum_k\nabla F(\mX^{(t)+k};\xi^{(t)+k})  	\\
%	\end{aligned}
%\end{equation}

%
%Note that except that we consider separate learning rate $\eta_c$ for local step and $\eta_s$ for communication, the update scheme on local steps is equivalent to GT when $\mW=\mI$. And we use the average of $K$ local steps to update the tracking variable during communication.


%The full detail of $K$-GT is summarized in Algorithm \ref{algo: k-gt}.
%\begin{savenotes}
\begin{algorithm}
	\caption{$K$\nobreakdash-GT: Gradient Sum 
Tracking}
\resizebox{\linewidth}{!}{
	\begin{minipage}{1.05\linewidth}
	\label{algo: k-gt}
	\begin{algorithmic}[1]
		\State \textbf{parameters:}
		 $T$: number of communication; $K$: number of local steps; $\eta_c,\ \eta_s$: local, communication stepsize; $\mW$: given topology.
		\State \textbf{Initialize:} $\forall i,j\in[n],\ \xx^{(0)}_i = \xx^{(0)}_j;\ \cc_i^{(0)}= - \nabla F_i(\xx^{(0)}; \xi_i)+\frac{1}{n}\sum_j\nabla F_j(\xx^{(0)}; \xi_j) $\footnote{This initialization in correction $\cc_i^{(0)}$ is required for heterogeneity-independent analysis in theory. We demonstrate later with experiment that simply choosing $\cc_i^{(0)} = \zero$ works well in practice.}.
		\For{client $i\in\{1,\ldots,n\}$ parallel}
			\For{\textbf{communication:} $t\gets0$ to $T-1$}
				\For{\textbf{local step:} $k\gets0$ to $K-1$}
					\State $\xx_i^{(t)+k+1} = \xx_i^{(t)+k} - \eta_c(\nabla F_i(\xx_{i}^{(t)+k}; \xi_i^{(t)+k}) + \cc_i^{(t)})$
				\EndFor
				\State $\zz_i^{(t)} = \tfrac{1}{K\eta_c}(\xx_i^{(t)} - \xx_i^{(t)+K})$
				\State $\cc_i^{(t+1)} = \cc_i^{(t)} - \zz_i^{(t)} + \sum_j w_{ij}\zz_j^{(t)}$ \Comment{update tracking variable}
				\State $\xx_i^{(t+1)} = \sum_jw_{ij}(\xx_j^{(t)}-K\eta_s\eta_c\zz_j^{(t)})$\Comment{update model parameters}
			\EndFor
		\EndFor
	\end{algorithmic}
\end{minipage}}
\end{algorithm}
%\end{savenotes}
%\vspace{-5mm}


%\begin{remark}
%	\label{remark: p}%SEB: p should go into the assumption\ldots
%  \ak{I think it is also required that $|w_{ij}| \leq 1$, otherwise $\rho$ might be bigger than 1. } The mixing rate describes the sparsity of communication graph. The larger value of $p$ means the communication graph is better connected. $p=1$ if complete graph $\mW = \tfrac{1}{n}\unit\unit^T$, and $p=0$ if identity matrix $\mW = \mI$.
%\end{remark}
\subsection{Main theorem: data-independent convergence on non-convex functions}
In this section, we present the convergence rate of $K$-GT. Note that $p$ is the network parameter defined in Assumption~\ref{ass:p}.
%Assumption~\ref{ass: mixing}.
%Remark~\ref{remark: p}.

\begin{theorem}[{$K$-GT convergence}]
\label{thm: k-gt}
For schemes as in Algorithm~\ref{algo: k-gt} with mixing matrices such as in Assumption \ref{ass:p} and arbitrary error $\epsilon>0$, there exists a constant stepsize $\eta_c=O(\frac{p}{KL})$ and $\eta_s=O(p)$ such that under Assumption \ref{ass:l} and \ref{ass:noise} for $L$\nobreakdash-smooth, (possibly non-convex) functions, it holds $\frac{1}{T+1}\sum_t\mE||\nabla f(\bar\xx^{(t)})||^2\leq \epsilon$ after $$\cO\left(\frac{\sigma^2}{Kn\epsilon^2} +\frac{\sigma}{p^2\sqrt{K} \epsilon^{\frac{3}{2}}}+\frac{1}{p^2 \epsilon}\right)\cdot L$$ communication rounds.
\end{theorem}
%SEB: \bar x is not define
%\vspace{-5mm}

%\begin{remark}Then when , $\mX^{(t)+0} \equiv \mX^{(t)}$, $K$\nobreakdash-GT is equivalent to the classical GT when $\eta=\eta_s\eta_c$.\end{remark}

%\item \textbf{Variance-reduced algorithm:} Consider rewriting the correction $\mC$, \begin{equation}\label{eq: k-gt, correction}\mC^{(t+1)} = \mC^{(t)}\mW + \frac{1}{K}\sum_k\nabla F(\mX^{(t)+k};\xi^{(t)+k})(\mW -\mI),\end{equation} it captures the direction difference between communicated model and local model, and corrects for the drift on every local step, which is similar to the variance-reduced framework in centralized optimization.
%And also we show that
%\begin{restatable}[Equivalence to SCAFFOLD]{proposition}{scaffold}
%\label{proposition: scaffold}
%	when the network topology is a complete graph, $K$\nobreakdash-GT is equivalent to a SVRG-like centralized algorithm SCAFFOLD~\citep{scaffold} with option II.
%\end{restatable}
%The SCAFFOLD algorithm is included in Appendix~\ref{ap: scaffold}.


\vspace{-5mm}
\section{Discussion}\label{sec: discuss}
In this section, we are going to introduce and compare with other possible ways of introducing local steps to GT that has the similar communication pattern as $K$\nobreakdash-GT.
%\subsection{Stochastic Gradient Tracking Framework.}
%

%The basic GT is in this framework with $\mG^{(t)}=\nabla F(\mX^{(t)}; \xi^{(t)})$ and $\mW^{(t)}=\mW$. Our method $K$\nobreakdash-GT could also fit in it with $\mG^{(t)} = \textstyle \sum_{k}\nabla F(\mX^{(t)+k};\xi^{(t)+k})$ and $\mW^{(t)}=\mW$.
\vspace{-5mm}
\subsection{Other GT alternatives}\label{sec:alternatives}


 \subsubsection{Gradient Tracking with Periodical Communication (Periodical GT).} \label{sec:perodical_gt}
 There is another way to incorporate local steps into above framework~(\ref{eq: dsgt}). Instead of communication via fixed topology $\mW$, the communication graph changes along with time denoted by $\mW^{(t)}$. Note that $\mW^{(t)} = \mI$, which means there is actually no communication. %$\mI$~(no communication, local steps) and $\mW$~(communication) and $\mG^{(t)}=\nabla F(\mX^{(t)}; \xi^{(t)})$.%, $$\mW^{(t)}=\bigg\{\begin{matrix}\mW & \mbox{mod($t, K$)}=0 \\\mI & else\end{matrix},$$ and $\mG^{(t)}=\nabla F(\mX^{(t)}; \xi^{(t)})$.
 If $\mW^{(t)}$ periodically alternates between $\{\mW,\ \mI\}$, it also reduces communication frequency. The full detail is concluded in Algorithm~\ref{algo: periodical_gt}~(Appendix~\ref{ap: periodical_gt}).
\vspace{-2mm}

\paragraph*{$K$\nobreakdash-GT suffers from less noise than Periodical GT.} It is possible to reformulate local steps of Periodical GT as corrected SGD, same as that for $K$\nobreakdash-GT. But Periodical GT has different update for correction at communication with
\begin{equation}
		\mC^{(t+1)}=\mC^{(t)}\mW + \nabla F(\mX^{(t)+K-1}; \xi^{(t)+K-1})(\mW-\mI)\,.
	\label{eq: tv_gt}
\end{equation} The equivalence of reformulation is proven in Appendix~\ref{ap: reformulation}.

However, if we simply reformulate equation (\ref{eq: k-gt}), we obtain that $K$\nobreakdash-GT uses the average of $K$ stochastic gradient, %SEB: I removed this link, as (B2) is about periodic-GT and not K-GT, this is confusing (and reference is only in appendix)
% in~(\ref{eq: k-gt, comm})
i.e., $$\mC^{(t+1)}=\mC^{(t)}\mW + \tfrac{1}{K}\textstyle\sum_k\nabla F(\mX^{(t)+k}; \xi^{(t)+k})(\mW-\mI)\,,$$ which can reduce stochastic noise by $K$. Periodical GT uses only one stochastic gradient, thus would suffer more from stochastic noise. %The detailed algorithm of Periodical GT is included in Alg.~\ref{algo: tv_gt2}~(Appendix~\ref{ap: periodical_gt}).

\paragraph*{Using more random samples on stochastic gradient can reduce noise in Periodical GT.}
 It is trivial to reduce the stochastic noise in~(\ref{eq: tv_gt}) if using more random samples $\{\xi^{(t),s}|s = 0,\ldots,K-1\}$ to replace $\nabla F(\mX^{(t)+K-1}; \xi^{(t)+K-1})$ with\begin{equation}\nonumber\nabla F(\mX^{(t)+K-1}; \xi^{(t)+K-1}) = \frac{1}{K}\sum_s\nabla F(\mX^{(t)+K-1}; \xi^{(t)+K-1,s})\,,\end{equation} then the correction $\mC^{(t)}$ has the same level of stochastic noise as $K$\nobreakdash-GT. However, using more sample to calculate SGD requires a lot more extra computation than $K$\nobreakdash-GT. %The Periodical GT using full gradient is shown in Alg.~\ref{algo: tv_gt3} in Appendix~\ref{ap: periodical_gt}.

\begin{theorem}[Periodical GT convergence]\label{thm: tv_gt}For schemes as in Algorithm~\ref{algo: periodical_gt}~(Appendix~\ref{ap: periodical_gt}) with mixing matrices such as in Assumption \ref{ass:p} and arbitrary error $\epsilon>0$, there exists a constant stepsize $\eta=O(\frac{p^2}{KL})$ such that under Assumption \ref{ass:l} and \ref{ass:noise} for $L$\nobreakdash-smooth, (possibly non-convex) functions, it holds $\frac{1}{T+1}\sum_t\mE||\nabla f(\bar\xx^{(t)})||^2\leq \epsilon$ after $$\cO\left(\frac{\sigma^2}{Kn\epsilon^2} +\frac{\sigma}{p^2 \epsilon^{\frac{3}{2}}}+\frac{1}{p^2 \epsilon}\right)\cdot L
$$ communication rounds.
Conversely, if we consider using the full-batch tracking Algorithm~\ref{algo: periodical_gt_grad}~(Appendix~\ref{ap: periodical_gt}), then the convergence rate can be improved to $$\cO\left(\frac{\sigma^2}{Kn\epsilon^2} +\frac{\sigma}{p^2\sqrt{K}\epsilon^{\frac{3}{2}}}+\frac{1}{p^2 \epsilon}\right)\cdot L \,.$$
\end{theorem}
\noindent Note that the latter result refers to full batch tracking which comes at additional computation cost each communication round (in contrast to $K$-GT).


% \ak{I think we can still obtain $\frac{\sigma}{\sqrt{TK}}$ convergence rate in the first term for this variant, as these stochastic gradients are still incorporated in $X$.}

\subsubsection{Gradient Tracking with Large Batch (Large-batch GT)}
%SEB: here the batch size is $K$, but in the appendix there is no K??
Apart from local training, large-batch training is also popular to achieve acceleration in distributed setting. Similar to Large-batch SGD, we calculate $\mG^{(t)} = \sum_k\nabla F(\mX^{(t)}; \xi^{(t), k})$ in~(\ref{eq: dsgt}) with $K$ \iid random samples, $\{\xi^{(t),k}|k = 0,\ldots,K-1\}$ and make $\mW^{(t)} = \mW$.  It is theoretically workable to improve the asymptotical communication rounds needed to reach the desired accuracy $\epsilon$ from $\cO\big(\frac{\sigma^2}{n\epsilon^2}\big)$~\citep{koloskova2021improved} to $\cO\big(\frac{\sigma^2}{nK\epsilon^2}\big)$, while remains heterogeneity-independent.% Then we can improve the stochastic noise\tao{what is the meaning of 'improving the stochastic noise?'} in Assumption~(\ref{ass: noise}) by $K$\tao{need to be more specific}. While $\mW^{(t)}=\mW$, it's workable\tao{somehow very weak?} to improve the asymptotical communication rounds needed to reach the desired accuracy $\epsilon$ from $\cO\big(\frac{\sigma^2}{n\epsilon^2}\big)$~\citep{koloskova2021improved} to $\cO\big(\frac{\sigma^2}{nK\epsilon^2}\big)$, while remains heterogeneity-independent.
%

We empirically show that Large-batch GT remains heterogeneity-independent and has the same communication performance as $K$\nobreakdash-GT ~(Figure~\ref{fig: simulation_convex},~\ref{fig: large}).  %However, it suffers from poorer generalization performance on DNN models~(Appendix~\ref{app: large}).


%\subsection{Preliminary: Decentralized Stochastic Gradient Tracking}
%We now present the classical GT algorithm. Decentralized stochastic gradient tracking (GT)~\citep{gt, koloskova2021improved} is proven to converge independent of data heterogeneity. The model update consists of two components: (i) model $\xx_i$ updates with tracking variable $\zz_i$, and (ii) tracking $\zz_i$ updates with stochastic gradient. The protocol can be compactly written in matrix notation as follows,
%\begin{equation}\label{eq: dsgt}
%	\begin{aligned}
%		\mX^{(t+1)} & = (\mX^{(t)}-\eta \mZ^{(t)})\mW                                        \\
%		\mZ^{(t+1)} & = \mZ^{(t)}\mW +\mG^{(t+1)} -\mG^{(t)},
%	\end{aligned}
%\end{equation}
%where $\mG^{(t)}=\nabla F(\mX^{(t)};\xi^{(t)}).$
%\ak{Define $\mG$ in the matrix notation section. }
%\ak{This theorem holds only asymptotically. Tn the current form need to include all the terms. Alternatively could just have one sentence commenting stochastic term of convergence. }
%\begin{theorem}[\cite{koloskova2021improved}]\label{thm: dsgt}
%When adopting appropriate constant stepsize, the optimal convergence rate of GT is asymptotically $\tilde{O}\bigg(\frac{\sigma}{\sqrt{nT}}\bigg)$ for L-smooth and non-convex function $f(\xx)$, where $T$ is the number of iteration.
%\end{theorem}




%\subsection{Connection to Variance-reduction framework}We show $K$\nobreakdash-GT can be rewritten as corrected SGD in variance-reduction framework.
%\begin{restatable}[Corrected SGD update]{proposition}{csgd}\label{cor: csgd}The tracking variable $\mZ^{(t)+k}$ is equivalent to the SGD compensated by this correction, $$\mZ^{(t)+k} = \nabla F(\mX^{(t)+k}; \xi^{(t)+k}) + \mC^{(t)}.$$The correction is constant throughout all local steps and is updated every communication as
%\begin{equation}\label{eq: k-gt, correction}
%	\begin{aligned}
%		\mC^{(t+1)} & = \mC^{(t)} + \frac{1}{K\eta_c}(\mX^{(t)}-\mX^{(t)+K})(\mW -\mI)	\\
%				  & = \mC^{(t)}\mW + \frac{1}{K}\sum_k\nabla F(\mX^{(t)+k};\xi^{(t)+k})(\mW -\mI)
%	\end{aligned}
%\end{equation}
% \ak{Define $\mC^{(t)}$. \\
% 	I think the rule for updating $X$ is wrong here, as nor $X^{(t) + k}$, nor $\mC^{(t)}$ have any information about  $\nabla F(\mX^{(t)+k}; \xi^{(t)+k})$ (that is only in $Z$). }
%\end{restatable}
%\begin{remark}
%The equation for $\mC$ could be rewritten as $$\mC^{(t+1)} = \mC^{(t)}\mW + \frac{1}{K}\sum_k\nabla F(\mX^{(t)+k}; \xi^{(t)+k})(\mW -\mI).$$
%\end{remark}



%\paragraph*{Connection to variance-reduction}


%Then we have successfully bridged two independently developed SCAFFOLD and GT with $K$\nobreakdash-GT shown in Figure~\ref{fig: algorithm flow}.
%\begin{enumerate}
%\item GT is a decentralized heterogeneity-correction algorithm that communicates for every update, i.e, $K=1$.
%\item $K$\nobreakdash-GT extents tracking from single gradient to gradient sum of multiple local steps $K>1$ shown in Proposition~\ref{cor: local_gt}. Thus it reduces the communication frequency by $K$ comparing to GT.
%\item When decentralized communication topology is complete graph, $K$\nobreakdash-GT is equivalent to SCAFFOLD.
%\end{enumerate}
%\begin{figure}[H]
%	\centering
%	\includegraphics[width=0.5\textwidth]{./figure/algorithm_flow.jpg}
%	\caption{How GT, $K$\nobreakdash-GT and SCAFFOLD are related to each other under different setting. When number of local steps $K=1$, $K$\nobreakdash-GT is equivalent to GT. When the communication topology is complete, $K$\nobreakdash-GT is equivalent to SCAFFOLD.}
%	\label{fig: algorithm flow}
%\end{figure}

% \ak{I think this could be moved to a separate section. suggestion for renaming : Extension of K-GT with Alternating Communication.}
%\subsubsection{$K$\nobreakdash-GT with Alternating Communication ($K$\nobreakdash-AGT)}
%While the classical GT tracking algorithm mitigates the challenge of data heterogeneity,
%it should be noted that this comes with the disadvantage that the communication overhead per round is twice as high compared to D\nobreakdash-SGD. This is due to the fact that the tracking parameters have to be communicated in addition to the parameters.

%In contrast, the communication efficiency of $K$-GT can be improved:\ %since the algorithm (provably) allows local steps, we can alternate the communication. That is,
%in every communication round we either perform only the parameter mixing (line 9 in Alg.~\ref{algo: k-gt}) or only the mixing of the tracking variables.
%We illustrate this in  Appendix~\ref{ap: k-agt} ($K$\nobreakdash-AGT) and measure the empirical performance of this variant in Section~\ref{sec:experiments} below.
%The convergence proof of this $K$-AGT follows the same template as the proof of our main Theorem~\ref{thm: k-gt}, and we omit it for conciseness.
%\vspace{-5mm}
%\yue{delete the section for alternating communication here, since it has never been proven and how it could be proven is still not clear.}
%We now consider further improving communication efficiency by reducing communication model size\tao{confusing sentence}. $K$\nobreakdash-GT needs both $\mX$ and $\mC$ to communicate via the same topology. This can be relaxed by allowing for two separate matrices $\mW_x$ and $\mW_c$.
%\begin{equation}\nonumber
%	\begin{aligned}
%		\mX^{(t+1)} &= (\mX^{(t)} - \eta_s(\mX^{(t)} - \mX^{(t)+K}))\mW_x\\
%		\mC^{(t+1)} &= \mC^{(t)} +\frac{1}{K\eta_c}(\mX^{(t)}-\mX^{(t)+K})(\mW_z-\mI)
%	\end{aligned}
%\end{equation}
%If only one of $\{\mW_x,\mW_c\}$ could be $\mW$~(commmunication) at each time~(the left is $\mI$), then only one of $\{\mX,\mC\}$ is transmitted in network.

%Also note that, the gradient sum tracking in Proposition~\ref{cor: local_gt} still holds as long as replacing $\mW$ with $\mW_x$ and $\mW_z=\mW_c$\tao{confused.}, respectively. Thus when $K=1$, alternating $K$\nobreakdash-GT is equivalent to alternating GT~\citep{koloskova2021improved}.


%We later show in numerical result that $K$\nobreakdash-GT performs much better in generalization performance than Periodical GT in Figure~\ref{fig: simulation} and Figure~\ref{fig: local_steps}.



%\subsubsection{Large-batch GT. } Instead of using local steps, we consider large-batch training to have the same communication efficiency. It's due that the stochastic noise asymptotically dominates the convergence of GT~\citep{koloskova2021improved}. If using $K$ \iid samples to calculate stochastic gradient, we could reduce the stochastic noise from $\sigma^2$ to $\sigma^2/K$, and it's workable to improve the leading term of GT from $\cO(\sigma^2)$ to $\cO(\frac{\sigma^2}{K})$.

%The situation can be easily generalized to mini-batches scenario where GT uses larger batch $B$ and $K$\nobreakdash-GT uses smaller batch $B_{loc}$ and $B=KB_{loc}$. We empirically show that Large-batch GT suffers from poorer generalization performance than its substitute with local steps on DNN models in Figure~\ref{fig: local_steps}, which is very similar to the discussion over Large-batch SGD and Local SGD in~\cite{largebatch}.
\vspace{-4mm }
\subsection{Convergence comparison}

We summarized the convergence rate for the related decentralized algorithms  in Table~\ref{tab: convergence}. In order to analyze the convergence for other methods that depend on data heterogeneity, there is an addition assumption to measure data heterogeneity~\cite{scaffold,unified-dsgd}.
%\vspace{-5mm}
\begin{table}[tb]
\caption{The comparison of communication rounds needed to reach target accuracy $\epsilon$ on non-convex functions. Our results on both $K$-GT, Periodical GT improve the rate of D-SGD in terms of heterogeneity parameter $\bar\zeta^2$(defined in Ass. \ref{ass:zeta}) when using local steps, and accelerates the rate of GT. }
	\centering
	\renewcommand{\arraystretch}{1.2}
	\resizebox{0.75\textwidth}{!}{
		\begin{tabular}{l|l|ll}		
			\toprule[1.1pt]
			\multicolumn{1}{l}{\textbf{Local steps}} &\multicolumn{2}{l}{\textbf{Algorithm}} & \textbf{Communication rounds}	\\\midrule[0.8pt]
			$K=1$ &\multicolumn{2}{l}{GT~\citep{koloskova2021improved}} & $\cO\Big(\frac{\sigma^2}{n \epsilon^2} +\frac{\sigma}{p^{\frac{3}{2}} \epsilon^{\frac{3}{2}}}+\frac{1}{p^2 \epsilon}\Big)$ \\\cline{1-4}
			\multirow{4}{*}{$K>1$}&\multicolumn{2}{l}{D\nobreakdash-SGD~\citep{unified-dsgd}} &$\cO\Big(\frac{\sigma^2}{Kn \epsilon^2} +(\frac{\bar\zeta}{p}+\frac{\sigma}{\sqrt{pK}})\frac{1}{\epsilon^{\frac{3}{2}}}+\frac{1}{p \epsilon}\Big)$ \\\cline{2-4}
			&\multicolumn{2}{l}{$K$\nobreakdash-GT {\textbf{[ours]}}}&  $\cO\Big(\frac{\sigma^2}{Kn \epsilon^2} +\frac{\sigma}{p^2\sqrt{K} \epsilon^{\frac{3}{2}}}+\frac{1}{p^2 \epsilon}\Big)$\\\cline{2-4}
			&\multicolumn{2}{l}{Periodical GT {\textbf{[ours]}}}&  $\cO\Big(\frac{\sigma^2}{Kn \epsilon^2} +\frac{\sigma}{p^2 \epsilon^{\frac{3}{2}}}+\frac{1}{p^2 \epsilon}\Big)$\\\cline{2-4}
			&\multicolumn{2}{l}{Periodical GT w/ full gradient {\textbf{[ours]}}}&  $\cO\Big(\frac{\sigma^2}{Kn \epsilon^2} +\frac{\sigma}{p^2\sqrt{K} \epsilon^{\frac{3}{2}}}+\frac{1}{p^2 \epsilon}\Big)$\\
			\bottomrule[1.1pt]
		\end{tabular}
		} %\vspace{-5mm}
\label{tab: convergence}		
\end{table}
%\iseb{what is $P$? (maybe state the rate for $P=0$ only), what is $\bar \zeta$?}, \iseb{the last two are also [ours] - but we need to make it more clear for which purpose we state these results in the table as well?}
\vspace{-2mm }
\paragraph*{$K$\nobreakdash-GT achieves acceleration by local steps in high-noise regime.} When $\epsilon$ is sufficiently small, the noise dominates the convergence rate ($\sigma>0$) and it is not affected by graph parameter $p$ for GT, Periodical GT and $K$\nobreakdash-GT. Then after enough transient time, Periodical GT and $K$\nobreakdash-GT with $\cO(\frac{\sigma^2}{nK\epsilon^2})$ achieves linear speedup by $K$ compared to GT with rate $\cO(\frac{\sigma^2}{n\epsilon^2})$.
In addition, the transient time for $K$\nobreakdash-GT also decreases with $\cO(\frac{1}{\sqrt{K}})$ comparing to GT baseline.

GT methods are in general more sensitive to the network parameter than diffusion methods~\citep{primal>primal-dual}, e.g., D\nobreakdash-SGD, in the non-asymptotical regime. In our analysis of $K$\nobreakdash-GT, the dependency on the network parameter $p$ is worse than for vanilla GT. Combining our analysis with the tighter analysis of GT presented in concurrent work~\cite{koloskova2021improved} would be an interesting future direction---however in this work we focused on the aspect of equipping GT with local steps.

\vspace{-2mm }
\paragraph*{The impact of data heterogeneity is removable for $K$\nobreakdash-GT .} %The leading terms are the same\tao{where is the rate for D-SGD with local steps?}. But
$K$-GT does not completely solve data heterogeneity in general, and depends on the data heterogeneity at the initial point, which is the same case in GT. It has been proven for GT that in the non-asymptotic regime a weaker dependence on the data heterogeneity at the initial point actually remains~\cite{koloskova2021improved}. However, with a single round of global communication for the initial iterates (e.g. in Alg.~\ref{algo: k-gt}), we can remove the heterogeneity from the complexity estimates for GT, $K$-GT and Periodical GT. Table~\ref{tab: convergence} removes the initialization terms from the rate to simplify the presentation. On the contrary, heterogeneity $\bar\zeta^2$ under no circumstance can be eliminated for D-SGD and slows down its convergence.

\vspace{-2mm }
\paragraph*{Periodical GT suffers more from noise comparing to $K$\nobreakdash-GT.} In asymptotical regime, the transient time for $K$\nobreakdash-GT $\cO(\frac{\sigma}{\sqrt{K}})$ decrease with local steps while Periodical GT $\cO(\sigma)$ does not. But this noise term can be improved as discussed in section~\ref{sec:perodical_gt}.  If we consider a full gradient in equation~(\ref{eq: tv_gt}), Periodical GT performs similar to $K$\nobreakdash-GT at the expense of extra computation.
%\vspace{-5mm}
\section{Experimental results}
\label{sec:experiments}
We evaluate the effectiveness of $K$-GT by comparing it with D-SGD and periodical GT.% and Large-batch GT\footnote{Large-batch GT to GT is  what Large-batch SGD is to SGD, considering using more batches when calculating stochastic gradient.} to show its superiority over other alternatives that also have potential to achieve acceleration.% , i.e., $\mG^{(t)}=\sum_{s=0}^{K-1}\nabla F(\mX^{(t)}; \xi^{(t), s})$ in (\ref{eq: dsgt}) instead of $\mG^{(t)}=\nabla F(\mX^{(t)};\xi^{(t)})$, where $\{\xi^{(t),s}|s = 0,\ldots,K-1,\ S>1\}$ are \iid drawn random samples. It's easy to show from the analysis~\citep{koloskova2021improved} that Large-batch GT also improves the asymptotical communication rounds needed to reach the desired accuracy $\epsilon$ from $\cO\big(\frac{\sigma^2}{n\epsilon^2}\big)$ to $\cO\big(\frac{\sigma^2}{nK\epsilon^2}\big)$ regardless of heterogeneity.
\vspace{-3mm}
\subsection{Setting}
We conduct experiments in two settings. 
\begin{enumerate}
	\item \textsc{Synthetic datasets:} We first construct the distributed least squares objective with $f_i(\xx)=\frac{1}{2}||\mA_i\xx-\bb_i||^2$ with fixed Hessian $\mA_i^2=\frac{i^2}{n}\cdot \mI_d$, and sample each $\bb_i\sim\cN(0,\frac{\bar\zeta^2}{i^2}\cdot\mI_d)$ for each client $i\in[n]$, where $\bar\zeta^2$ can control the deviation between local objectives~\citep{unified-dsgd}. Stochastic noise is controlled by adding Gaussian noise with $\sigma^2=1$.  
	\item \textsc{Real-world dataset, mnist~\cite{mnist}}: We test the case that all clients collaboratively train a convolutional neural network~(CNN)\footnote{Here we only consider a very simple network without Batch Norm layers~\citep{batchnorm} for simplicity, since it inherently assumes that the data distribution is uniform across different batches, which is not the case that we are interested in. The detailed network structure is listed in Appendix~\ref{appendix: network}.} on real-world dataset, \textsc{mnist}. In total this dataset contains 60,000 images of size 28×28 and 10 labels. \end{enumerate}
We use a ring topology for both sets of experiments. For simplicity, instead of using the initialization in Alg.~\ref{algo: k-gt}, we initialize $\cc_i=\zero$ for all experiments.%footnote{In fact, all $\zero$'s intialization for correction $\cc_i^{(0)}$ won't affect the performance in practice.}.
%
For data partition on \textsc{mnist}, we consider both homogeneous and heterogeneous cases. The homogeneous dataset is first shuffled and then
uniformly partitioned among all the clients. We call this the `random' setting. The heterogeneous datasets is created when each client only has exclusive access to subset of classes. We call this the `sorted' case, and the data variation across clients is maximized at this time. We use $n=5$ and $n=10$ clients and each client has access to one and two classes case accordingly, and the case $n=10$ has more severe heterogeneity condition than the case $n=5$.
\vspace{-4mm }
\paragraph*{Parameter tuning.} For \textsc{Synthetic datasets}, we use the same learning rate $\eta_s$=1 and $\eta$=1e-3. For \textsc{mnist}, we use the best constant learning rate tuned from $\{$0.5, 0.1, 0.05, 0.01, 0.005, 0.001$\}$ for algorithms and batch size 128 on each client. Note that even though our algorithm is purposed with constant learning rate, using more sophisticated and time-varying learning rate scheduler would definitely bring much better performance. 
\vspace{-4mm }
\paragraph*{Comparison.} We mainly illustrate the acceleration and robustness in convergence rate of the $K$\nobreakdash-GT compared to baseline D\nobreakdash-SGD. We also consider the performance of several GT-variants that supports local steps discussed in Section~\ref{sec: discuss}. 

\vspace{-2mm }
\subsection{Numerical results}
\begin{figure}
	\centering
	\includegraphics[width=1\textwidth]{./figure/simulation.pdf}
	\caption{Training \textbf{\textsc{synthetic}} convex functions over ring by 10 clients with noise $\sigma^2 = 1$. In total 5000 communication rounds for $K=1$~(top row) while only 250 rounds for $K=20$~(bottom row). All uses the same learning rate and are averaged by three repetitions. The client\nobreakdash-drift for D\nobreakdash-SGD is even more severe with increasing heterogeneity~(larger $\bar\zeta$) as well as $K$. $K$\nobreakdash-GT, GT, and GT w/ full grad are consistent for different $\bar\zeta^2$ while achieving communication reduction when $K>1$.  }
	\label{fig: simulation_convex}
\end{figure}

\begin{figure}
	\begin{subfigure}{0.5\textwidth}
		\centering
  		\includegraphics[width=1\textwidth]{./figure/k_1.pdf}
		\caption{$K=1$, and data is partitioned either random or sorted.}
		\label{fig: baseline}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.5\textwidth}
		\centering
  		\includegraphics[width=1\textwidth]{./figure/k_1e.pdf}
		\caption{$K=\tfrac{1}{n}$ epoch, and data is partitioned sorted. }
		\label{fig: local_steps}
	\end{subfigure}
	\caption{{Generalization performance} on \textbf{\textsc{mnist}} among D\nobreakdash-SGD~(blue), $K$\nobreakdash-GT(red), GT w/o~(orange) and w/~(green) full gradient for $n=5$~(top row) and $n=10$~(bottom row) clients. The $x$-axis corresponds to (a) the number of pass over overall dataset(epoch), and (b) the number of communication rounds. % Large-batch~GT(purple).  
	In (a), when $K=1$, $K$-GT and Periodical GT are identical to GT baseline~(remark \ref{remark: equivalence}). 
	Learning rates are tuned to be the best. Note that 1~epoch of passing over global dataset is equivalent to 470 times computation on SGD when mini-batch sized 128. And for (b), since $nK=470$ is fixed for both $n=5$~(top right) and $n=10$~(top left), the number of local steps between communication rounds is $K_{n=5} = 2K_{n=10}$.}%Only $K$\nobreakdash-GT and $K$\nobreakdash-AGT recovers the performance in baseline for different heterogeneity. D\nobreakdash-SGD and Periodical GT are suffering from 'client-drift' in DNN models.   }%from $\eta=\{2, 1, 0.5,0.1,0.05,0.01,0.005,0.001\}$ for all experiment. }
	\label{fig: mnist}
\end{figure}

\paragraph*{$K$-GT is the most robust against heterogeneity.} In the convex case, client drift only happens for D\nobreakdash-SGD suggested by Figure~\ref{fig: simulation_convex} in which the larger value $\bar\zeta^2\neq 0$ gets, the poorer model quality D\nobreakdash-SGD ends up with. However, $K$\nobreakdash-GT, Periodical GT (w/ and w/o full grad) and Large\nobreakdash-batch GT do not suffer from 'client\nobreakdash-drift' and ultimately reach the consistent level of model quality regardless of increasing of $\bar\zeta$ and $K$ (number of either local steps or random samples). % and number of local steps $K$. 
In the non-convex case, since it's known the optimality condition and optimization trajectory is more complex than the convex case, generalization performance of all methods in Figure~\ref{fig: mnist} cannot fully recover the baseline performance when data partition is random.  However, $K$-GT could always outperform when data partition is non-\iid and the improvement is more significant when the degree of heterogeneity is increasing from Figure~\ref{fig: local_steps}.


\paragraph*{Local step reduces communication. } From $K=1$ to $K=20$ in Figure~\ref{fig: simulation_convex}, $K$\nobreakdash-GT and other GT alternatives reach the same target after 2000 rounds to only 100 rounds, achieving linear reduction in communication with the help of local steps. However, more local steps makes D\nobreakdash-SGD suffer even more in model quality. At the same time, introducing local steps into the training of non-convex functions would still achieve communication reduction but not by a linear factor of $K$ as in the convex case. Within Figure \ref{fig: local_steps}, we fixe $nK=1$ epoch over the data such that for no matter which $n=5$ or $n=10$ client communicates once after 1 epoch of computation. Compared to $K=1$ in Figure~\ref{fig: simulation_convex}, the acceleration when $K>1$ is still by a huge amount. However, note that introducing more local steps when data partition is heterogeneous would result in more severe quality loss, but $K$-GT still outperforms. % \ak{Inconsistency: In the discussion above, Periodical GT didn't have any client\nobreakdash-drift, but was suffering from the worse noise reduction. }


\paragraph*{Large-batch GT has similar performance to tracking with local steps.} From both convex~(Figure~\ref{fig: simulation_convex}) and non-convex~(Figure~\ref{fig: large}) functions, either $K$-GT or Large-batch GT, after the same number of communication rounds while the simultaneously the same number of computation epochs, reaches the similar level of accuracy. But for D-SGD, training with local steps could be even more stable and generalizes better than the Large-batch, which has been empirically investigated in~\citep{largebatch}.

%\subsubsection*{Non-convex functions}
%In addition, we also construct a distributed non-convex objective with $f_i(\xx) = \frac{1}{2}||a_i\prod_j^d\xx^j - b_i||_F^2$  where $\xx^j$ is the $j$-th coordinator of vector $\xx\in\mathbb{R}^d$~($d$>1) and $a_i = \frac{i^2}{n}\in\mathbb{R}$, and $b_i\in\mathbb{R}$ is sampled from $\cN(0,\frac{\bar\zeta^2}{i^2})$. The deviation between local objectives could also be controlled by varying $\bar\zeta^2$. %Training non-convex function with stochastic noise is unstable\tao{maybe we should include too many details. the results are anyway unsatisfactory}, since there might be multiple stationary points for a non-convex function, and stochastic noise could help the optimization suddenly jump out of the neighborhood of a local optimum. Then it's hard to measure the optimization quality with just gradient norm $||f(\bar\xx)||^2$. %
%For simplicity, we set the scale of stochastic noise to $\sigma^2 =0$ and use the same learning rate $\eta_s$=1 and $\eta$=1e-3 for $K$-GT, Periodical GT and D-SGD\footnote{Without the concern of stochastic noise, Periodical GT is identical to Periodical GT with full gradient. And since Large-batch training is a technique of noise reduction, Large-batch GT is not considered either.} in Figure~\ref{fig: simulation_nonconvex}.



%Suggested by the theory, in order to show only the impact of data heterogeneity on the convergence of gradient norm, we don't consider any stochastic noise, $\sigma^2 =0$ in Figure~\ref{fig: simulation_nonconvex}. Also shown from Table~\ref{tab: convergence}, the heterogeneity parameter appears in the rate of D-SGD independent of stochastic noise, then the larger degree of heterogeneity still slows down the convergence of D-SGD but has no impact on $K$-GT and Periodical GT if we train models without any noise.  We use the same learning rate $\eta_s=1$ and $\eta=1e-3$ for only $K$-GT, Periodical GT and D-SGD\footnote{Without the concern of stochastic noise, Periodical GT is identical to Periodical GT with full gradient. And since Large-batch training is a technique of noise reduction, there is also no need to consider Large-batch GT.} in Figure~\ref{fig: simulation_nonconvex}.
%\begin{figure}[tb]
%	\centering
%\includegraphics[width=0.8\textwidth]{./figure/simulation_nonconvex_grad.pdf}
%	\caption{Training simulated non-convex functions over ring by 5 clients without noise. In total 10000 communication rounds for $K=1$~(above row) while 500 rounds for $K=20$~(below row). All uses the same learning rate  $\eta_s$=1 and $\eta$=1e-3 and are averaged by three repeitition. Only the convergence of D-SGD from bottom right is negatively impacted by $\bar\zeta^2$ while others perform consistently regardless of local steps.}
%	\label{fig: simulation_nonconvex}\vspace{-3mm}
%\end{figure}

%\textbf{$K$-GT achieves linear speed up in communication without the loss of performance on heterogeneous data. } Even though the optimization trajectory is different\footnote{Please note that even though we train model under different heterogeneity with the same model initialization $\xx^{(0)}$, it's easy to check that even the centralized gradient $\sum_if_i(\xx^{(0)}; b_i)$ is different from the beginning for $\bar\zeta^2$=0 and =100 in simulation construction. Unlike the guarantee of sufficient decrease in strongly convex functions in Figure~\ref{fig: simulation_convex}, it's reasonable that the optimization trajectory for different $\bar\zeta^2$ is very different in Figure~\ref{fig: simulation_nonconvex}. } under different $\bar\zeta^2$, we could still compare methods under the same $\bar\zeta^2$ when using different choice of local steps to illustrate the impact of heterogeneity. In Figure~\ref{fig: simulation_nonconvex}, the convergence of D\nobreakdash-SGD is heavily negatively impacted by data heterogeneity indicated by the bottom right plot. For the same degree of heterogeneity, $K$\nobreakdash-GT and Periodical GT are consistent for different choice of number of local steps. The more local steps are used, the more communication reduction is achieved.
%\vspace{-5mm}
%\subsection{CIFAR-10 dataset}
%We further compare performance on ring of CIFAR\nobreakdash-10~\citep{cifar10} with ResNet-8~\citep{resnet}. Heterogeneous data is created via dirichlet distribution into 8 disjoint clients~\citep{non-iid-benchmark}.
%\begin{wrapfigure}{R}{6cm}
%	\centering
 % 	\includegraphics[width=0.45\textwidth]{./figure/5epoch.pdf}
%	\caption{Generalization performance of ResNet-8 on CIFAR10 under heterogeneous data. Local steps $K=5$ epochs.  }%from $\eta=\{2, 1, 0.5,0.1,0.05,0.01,0.005,0.001\}$ for all experiment. }
%	\label{fig: cifar10}
%\end{wrapfigure}
%\vspace{-2mm}

%\textbf{$K$\nobreakdash-GT always restores the best performance and achieves acceleration with local steps.} Figure~{\ref{fig: baseline}} shows the baseline of D\nobreakdash-SGD and GT for different heterogeneity when there is not any local steps. Unlike on the linear models in the previous simulation result, GT is not ideally independent of heterogeneity on DNN models like ResNet as suggested by its theory, which has been empirically observed by~\cite{lin2021quasi}, even though it still performs better than D\nobreakdash-SGD. Despite that GT's performance slightly degrades with severer heterogeneity, only $K$\nobreakdash-GT could always recover the corresponding baseline when using local steps, but needs much less communication overhead.

%\textbf{Periodical GT fails on DNN models.} Periodical GT, suffers from even worse `client\nobreakdash-drift' than D\nobreakdash-SGD on DNN models in Figure~\ref{fig: cifar10}. Full gradient calculation alleviates the drift to some extent, but it's still not satisfactory. In fact, the use of full gradient makes Periodical GT very likely to SVRG~\citep{svrg}
%, d-svrg, network-svrg}
%. Since we focus on the generalization performance for a DNN model with Batch Norm~\citep{batchnorm}, even in the non-distributed setting, training SVRG in this case is troublesome~\citep{ineffect-svrg}.

%\textbf{Alternating communication does not affect performance.} Figure~\ref{fig: cifar10} shows
% different mixing matrices for $\mW_x,\mW_z$ in
%that using alternating parameter/tracking mixing ($K$\nobreakdash-AGT) does not result in significant quality loss compared to $K$\nobreakdash-GT, but reducing half of the communication load.

%\paragraph*{Baseline.} We consider the base performance of D\nobreakdash-SGD and GT without local steps, since communication is the most sufficient this time. Note that $K$\nobreakdash-GT and Periodical GT are equivalent to GT when $K=1$.
% \ak{mention in the text explicitly which algorithm did you run on these graphs. }
%Figure~\ref{fig: baseline} shows the generalization performance of GT is not ideally independent of heterogeneity in DNN models as in theory, which has been empirically observed by~\cite{lin2021quasi}.
% \ak{This is counter-intutitive to me. GT should be not affected by heterogeneity. }

%\paragraph*{Local steps. }Then we first consider how the performance is affected by local steps. In Figure~\ref{fig: local_steps}, it's observed only $K$\nobreakdash-GT could be able to restore the best result in baseline after having local steps. D\nobreakdash-SGD drifts more with increasing heterogeneity.
%More systematic analysis for ResNet are discussed in Appendix~\ref{app: cifar10}.


%\textbf{Large-batch tracking cannot generalize well.} In practice of distributed training,  using batch size $B_{\mbox{loc}}$ on each local steps and using larger batch like $KB_{\mbox{loc}}$ but no local step are supposed to have similar communication performance. %Then we consider the result between using Large-batch and using local steps.
%However, different from consistent performance on convex functions~(Figure~\ref{fig: simulation}), Figure~\ref{fig: large_batch} shows that using local steps in $K$\nobreakdash-GT has much better generalization performance than Large-batch GT on such DNN models, which is similar to the discussion between Large-batch SGD and Local SGD in~\citep{largebatch}.



%\paragraph*{Alternating Communication. }Finally, in Figure~\ref{fig: local_steps}, we observe
% different mixing matrices for $\mW_x,\mW_z$ in that using alternating parameter/tracking mixing ($K$\nobreakdash-AGT) does not result in significant quality loss compared to $K$\nobreakdash-GT, but reducing half of the communication load.
\begin{figure}%{r}{6cm}
	\centering
	%\vspace{-2cm}
  	\includegraphics[width=0.3\textwidth]{./figure/large.pdf}
	\caption{{Generalization performance comparison} on \textbf{\textsc{mnist}} between large-batch training and training with local steps, where large-batch training uses $KB_{loc}$ local batch size and communicates every update, while training with local steps uses $B_{loc}$ local batch size and communicates periodically every $K$ local update.}%from $\eta=\{2, 1, 0.5,0.1,0.05,0.01,0.005,0.001\}$ for all experiment. }
	\label{fig: large}
\end{figure}

\vspace{-4mm }
\section{Conclusion}
Decentralized learning is a promising building block for the democratization of Deep Learning.
Especially in Edge AI applications, users' data does not follow a uniform distribution. This requires
robustness of decentralized learning algorithms to data heterogeneity.

%We address solve for heterogeneity impact on decentralized stochastic optimization with local steps.
We propose a novel decentralized optimization algorithm ($K$\nobreakdash-GT) supports communication efficient local update steps and overcomes data dissimilarity.
% by extenting gradient tracking to gradient sum tracking.
The tracking mechanism uses the accumulated gradient sum, akin to momentum, thereby reducing variance across local updates without the need of large batch sizes.
We demonstrated the superiority of $K$\nobreakdash-GT with both convergence guarantees and empirical evaluations. %compared to other GT-variants.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
%\bibliographystyle{plain}
\bibliographystyle{tfs}
\bibliography{reference}
%\input{main.bbl}%SEB: needed to hardcode this, as bibtex is not working on the submission server
\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\appendix
%\addcontentsline{toc}{section}{Appendix}
%\parttoc
%\begin{appendices}
\newpage
\appendix

%% SEB: I had to comment this out to make it compile
%% -------------------------------------------------
%\DoToC
%\renewcommand\contentsname{\normalsize \textbf{Contents of Appendix}}
%\contentsname
%\hypersetup{linkcolor=black}
%\startcontents[section]

%\printcontents[section]{l}{0}{\setcounter{tocdepth}{2}}
%
\hypersetup{linkcolor=red}
\setcounter{page}{1}

\input{appendix.tex}
\input{others.tex}
%\input{algorithm.tex}
%\input{periodical_gt.tex}
%\input{others.tex}



==> journal/others.tex <==
\onecolumn
\section{Experimental details}\label{appendix: network}
\subsection{Visualization of benchmark datasets}
\begin{figure}[H]
	\begin{subfigure}[t]{0.15\textwidth}
		%\centering
  		\vspace{12pt}
		\includegraphics[width=1\textwidth]{./figure/mnist.png}
		\caption{}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.85\textwidth}
		%\centering
  		\vspace{0pt}
		\includegraphics[width=1\textwidth]{./figure/data.pdf}
		\caption{}
	\end{subfigure}
	\caption{Data visualization. (a) Example from \textsc{mnist} dataset. (b) Data partition on each node in the random and the sorted case when there are $n=10$ distributed nodes. The dot size indicates the number of samples per class allocated to each node. }
\end{figure}

We show an image example from \textsc{mnist} datasets and how data of different labels is partitioned in random and sorted case. It obviously presents in the random case, data of different labels are randomly and evenly partitioned among nodes, but in the sorted case, each node only contains images of 1 label and the labels obtained by each node is non-overlapping.
\subsection{Model structure}
For our non-convex experiment, we use a 4-layer Convolutional Neural
Network (CNN) and its details are listed in Table~\ref{tab: network}.
\begin{table}[H]
\caption{Model architecture of the benchmark experiment. For convolutional layer (Conv2D), we
list parameters with sequence of input and output dimension, kernal size, stride. For
max pooling layer (MaxPool2D), we list kernal and stride. For fully connected layer (FC), we list
input and output dimension. For drop out (Dropout), we list the parameter of probability.}
	\centering
	\renewcommand{\arraystretch}{1.2}
	\resizebox{0.75\textwidth}{!}{
		\begin{tabular}{l|l}		
			\toprule[1.1pt]
			layer & details			\\\hline
			1 & Conv2D(1, 10, 5, 1), MaxPool2D(2), ReLU	\\
			2 & Conv2D(10, 10, 5, 1), Dropout2D(0.5), MaxPool2D(2), ReLU	\\
			3 & FC(320, 50), ReLU	\\
			4 & FC(50, 10)	\\
			\bottomrule[1.1pt]
		\end{tabular}}
		 %\vspace{-5mm}
\label{tab: network}		
\end{table}
